A Critical Review of Physics-Informed Machine Learning Applications in Subsurface Energy Systems

Machine learning has emerged as a powerful tool in various fields, including computer vision, natural language processing, and speech recognition. It can unravel hidden patterns within large data sets and reveal unparalleled insights, revolutionizing many industries and disciplines. However, machine and deep learning models lack interpretability and limited domain-specific knowledge, especially in applications such as physics and engineering. Alternatively, physics-informed machine learning (PIML) techniques integrate physics principles into data-driven models. By combining deep learning with domain knowledge, PIML improves the generalization of the model, abidance by the governing physical laws, and interpretability. This paper comprehensively reviews PIML applications related to subsurface energy systems, mainly in the oil and gas industry. The review highlights the successful utilization of PIML for tasks such as seismic applications, reservoir simulation, hydrocarbons production forecasting, and intelligent decision-making in the exploration and production stages. Additionally, it demonstrates PIML's capabilities to revolutionize the oil and gas industry and other emerging areas of interest, such as carbon and hydrogen storage; and geothermal systems by providing more accurate and reliable predictions for resource management and operational efficiency.

==> figures/activations.tex <==
\begin{subfigure}[b]{0.24\textwidth}
	\resizebox{\linewidth}{!}{%
		\begin{tikzpicture}
		\begin{axis}[ 
%title=$\tanh(x)$,
		xmin=-4, xmax=4,ymin=-2, 
		ymax=2, grid=major,
		height=5cm, width=5cm,
		axis line style={latex-latex},
		axis lines=middle,
		ticklabel style={font=\footnotesize,fill=white},
		minor tick num=1,
		scaled ticks=false] 
		\addplot[samples=100,red,very thick] {tanh(x))};
		%\addlegendentry{$\tanh(x)$}
		\end{axis}
	\end{tikzpicture} 
	}%
\subcaption{tanh}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.24\textwidth}
	\resizebox{\linewidth}{!}{%
	\begin{tikzpicture}
	\begin{axis}[ 
	%title=$\tanh(x)$,
	xmin=-4, xmax=4,ymin=-2, 
	ymax=2, grid=major,
	height=5cm, width=5cm,
	axis line style={latex-latex},
	axis lines=middle,
	ticklabel style={font=\footnotesize,fill=white},
	minor tick num=1,
	scaled ticks=false] 
	\addplot[samples=100,red,very thick] {1/(1+exp(-x))};
	%\addlegendentry{$\tanh(x)$}
	\end{axis}
	\end{tikzpicture}
	}%
	
\subcaption{sigmoid}
\end{subfigure}
\hfill
	\begin{subfigure}[b]{0.24\textwidth}
		\resizebox{\linewidth}{!}{%
		\begin{tikzpicture}
		\begin{axis}[ 
		%title=$\tanh(x)$,
		xmin=-4, xmax=4, ymin=-2, ymax=2, grid=major,
		height=5cm, width=5cm,
		axis line style={latex-latex},
		axis lines=middle,
		ticklabel style={font=\footnotesize,fill=white},
		minor tick num=1,
		scaled ticks=false] 
		\addplot[samples=100,red,very thick] {max(0,x)};
		%\addlegendentry{$\tanh(x)$}
		\end{axis}
		
		\end{tikzpicture}
}%
\subcaption{ReLU}
	\end{subfigure}
\hfill
		\begin{subfigure}[b]{0.24\textwidth}
			\resizebox{\linewidth}{!}{%
		\begin{tikzpicture}
		\begin{axis}[ 
		%title=$\tanh(x)$,
		xmin=-4, xmax=4,ymin=-2, 
		ymax=2, grid=major,
		height=5cm, width=5cm,
		axis line style={latex-latex},
		axis lines=middle,
		ticklabel style={font=\footnotesize,fill=white},
		, xticklabel style={anchor=north},
		minor tick num=1,
		scaled ticks=false] 
		\addplot[samples=100,red,very thick] {x/(1+exp(-x))};
		%\addlegendentry{$\tanh(x)$}
		\end{axis}
		
		\end{tikzpicture}
		}%
		\subcaption{Swish}
		\end{subfigure}


==> figures/stats.tex <==
\begin{tikzpicture}
    \begin{axis}[
        ybar,
        bar width=0.5cm,
        width=9cm,
        height=6cm,
		nodes near coords, % this command is used to mention the y-axis points on the top of the particular bar.
    nodes near coords align={vertical},
   %     xlabel={Domains},
        ylabel={Numnber of publications},
       % title={Bar Plot Example},
        xtick=data,
		ytick={0, 10, 20, 30, 40, 50, 60},
		xticklabels={Geoscience, Drilling, Reservoir, Production, CO\textsubscript{2} storage},
        ymajorgrids=true,
        grid style=dashed,
        ymin=0,
		ymax=60,
		ticklabel style = {font=\scriptsize}
    ]
    
    \addplot[fill=blue!50!white] coordinates {(1, 24) (2, 6) (3, 49) (4, 10) (5, 9)};
   % \addplot[fill=red] coordinates {(1, 3) (2, 4) (3, 8) (4, 6)};
    
    %\legend{Data 1}
    \end{axis}
    \end{tikzpicture}


==> sections/potential.tex <==
\section{Areas of potential research}
\label{section:potential}

Looking at table \ref{table:summary}
\citet{Yan2022b} interesting case


==> summary_backup <==

\begin{table}[ht]
\begin{center}
\rowcolors{1}{}{lightgray}
\begin{tabular}{p{11em}p{\textwidth/8}p{\textwidth/8}p{\textwidth/8}p{\textwidth/8}p{\textwidth/8}p{\textwidth/8}}
	 &  Data and\newline feature\newline engineering & Transfer\newline learning & Architecture\newline design &Loss function & Output \\\hline
	Geoscience&  \cite{Song2020} \cite{Alkhalifah2020} \cite{binWaheed2020}   &                   &\cite{McAliley2021} \cite{binWaheed2022} \cite{Cheng2022}& \cite{Alkhalifah2020b} \cite{Song2020} \cite{Song2021} \cite{Gou2023} \cite{Voytan2020} \cite{Moseley2020} \cite{Kumar2020} \cite{Alkhalifah2021} \cite{Huang2022} \cite{YijieZhang2023}	&  \\
	Drilling & \cite{Kharazmi2021}\cite{Kaneko2023}& \cite{Tang2022}                   &   \cite{Kharazmi2021}    \cite{Prasham2022}        & \cite{Tang2022} &        \\
	Petrophysics &   \cite{Yoga2022}   &                   & \cite{Tembely2021} \cite{Wu2018} &            &        \\
	\textbf{Reservoir engineering } &     &                   &   &            &        \\
	\hspace{.2in}Fluid flow	&      & &\cite{Maucec2022} \cite{Battaglia2016} \cite{KaiZhang2022}      \cite{ZhaoZhang2022} &  \cite{Fuks2020} \cite{Magzymov2021} \cite{Gasmi2021} \cite{Alhubail2022}\cite{ZhaoZhang2022} \Citep{Sambo2021} \Citep{Shen2022} &        \\
	\hspace{.2in}Waterflooding&      &                   &  \Citep{Liu2023}           &  &        \\
	\hspace{.2in}CO\textsubscript{2} storage &      &                   & \cite{Yan2022}&  &     \cite{Yan2022} \\
	\hspace{.2in}Reservoir modeling		&    \cite{Zhang2021}  &     \cite{Hadjisotiriou2023}              & \cite{Zhang2021}              &    \cite{Ihunde2021} \cite{Behl2023}\Citep{Wu2023}  & \cite{Wang2022}\Citep{Chen2023} \\
	Production forecasting	& \cite{Nagao2023} \cite{Manasipov2023} \cite{Staff2020} \cite{Razak2021c}   &  \cite{Razak2022}                  &   \cite{WendiLiu2023}\Citep{Darabi2022} \cite{Razak2022}        & \cite{Nagao2023}  \cite{WendiLiu2023} &\\\hline
\end{tabular}
\caption{Summary of papers using various PIML approaches per area of research. Instead of a category for hybrid models, works with several integration modes are classified into the different corresponding categories for the sake of clarity.}
\label{table:summary}
\end{center}
\end{table}

